Information Theoretic Model Predictive Q-Learning

Model-free Reinforcement Learning (RL) works well when experience can be collected cheaply and model-based RL is effective when system dynamics can be modeled accurately. However, both assumptions can be violated in real world problems such as robotics, where querying the system can be expensive and real-world dynamics can be difficult to model. In contrast to RL, Model Predictive Control (MPC) algorithms use a simulator to optimize a simple policy class online, constructing a closed-loop controller that can effectively contend with real-world dynamics. MPC performance is usually limited by factors such as model bias and the limited horizon of optimization. In this work, we present a novel theoretical connection between information theoretic MPC and entropy regularized RL and develop a Q-learning algorithm that can leverage biased models. We validate the proposed algorithm on sim-to-sim control tasks to demonstrate the improvements over optimal control and reinforcement learning from scratch. Our approach paves the way for deploying reinforcement learning algorithms on real systems in a systematic manner.

==> inputs/acknowledgments.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> inputs/related_work.tex <==
% !TEX root = ../bhardwaj20.tex
\vspace{-2mm}
\section{Related Work}\label{sec:related_work}
\vspace{-2mm}
% Model predictive control has a rich history in robotics, ranging from control of mobile robots such as quadrotors~\citep{desaraju2016fast} and aggressive autonomous vehicles~\citep{williams2017information,wagener2019online} to generating complex behaviors for high-dimensional systems such as contact-rich manipulation~\citep{kumar2014real,fu2016one} and humanoid locomotion~\citep{erez2013integrated}. The success of MPC can largely be attributed to online policy optimization which helps mitigate model bias. The information theoretic view of MPC aims to find a policy at every timestep that minimizes the cost over a finite horizon as well as the KL-divergence with respect to a prior policy usually specified by the system's passive dynamics~\citep{theodorou2012relative, williams2017information}. This helps maintain exploratory behavior and avoid over-commitment to the current estimate of the cost function, which is biased due to modeling errors and a finite horizon. Sampling-based MPC algorithms~\citep{williams2017information,wagener2019online} are also highly parallelizable enabling GPU implementations that aid with real-time control. However, efficient MPC implementations still require careful system identification and extensive amounts of manual tuning.
% Model predictive control has a rich history in robotic control, ranging aggressive autonomous driving~\citep{williams2017information,wagener2019online} to contact-rich manipulation~\citep{kumar2014real,fu2016one} and humanoid locomotion~\citep{erez2013integrated}. The information theoretic view of MPC aims to find a policy that minimizes the cost over a finite horizon as well as the KL-divergence with respect to a prior policy usually specified by the system's passive dynamics~\citep{theodorou2012relative}. This helps maintain exploratory behavior and avoid over-commitment to the current biased estimate of the cost function, due to model errors and finite horizon. Sampling-based algorithms~\citep{williams2017information,wagener2019online} are highly parallelizable enabling real-time GPU implementations. However, efficient MPC implementations still require careful system identification and extensive manual tuning.

% Deep RL methods are extremely general and can optimize neural network policies from raw sensory inputs with little knowledge of the system dynamics. Both value-based and policy-based approaches~\citep{schulman2015trust} have demonstrated excellent performance on complex control problems. These approaches, however, fall short on several accounts when applying them to a real robotic system. First, they have high sample complexity, potentially requiring millions of interactions with the environment. This can be very expensive on a real robot, not least because the initial performance of the policy can be arbitrarily bad. Using random exploration methods such a $\epsilon$-greedy can further aggravate this problem. Second, a value function or policy learned entirely in simulation inherits the biases of the simulator. Even if a perfect simulation is available, learning a globally consistent value function or policy is an extremely hard task as noted in~\citep{silver2016mastering,zhong2013value}. This can be attributed to local optima when using neural network representations or the inherent biases in the Q learning update rules~\citep{fox2015taming, van2016deep}. In fact, it can be difficult to explain why Q-learning algorithms work or fail~\citep{schulman2017equivalence}.  

% Model-free deep RL methods are extremely general and can optimize neural network policies from raw sensory inputs and have demonstrated excellent performance on complex control problems ~\citep{schulman2015trust}. However, they face several challenges when used on real systems. First, model free RL has high sample complexity, potentially requiring millions of interactions with the environment. This can be very expensive on a robot, as the initial performance of the policy can be arbitrarily poor. Using random exploration such a $\epsilon$-greedy policy can also be detrimental. Second, a value function or policy learned entirely in simulation inherits the biases of the simulator. Even if a perfect simulation is available, learning a globally consistent value function or policy is an extremely hard task as noted in~\citep{silver2016mastering,zhong2013value} due to local optima when using neural networks or the inherent biases in the Q learning update rules~\citep{fox2015taming, van2016deep}. Using these insights, we build our approach to leverage the complimentary strengths of model-based and model-free methods while mitigating their weaknesses.


% Domain randomization aims to make policies learned in simulation more robust by randomizing simulation parameters during training with the aim of making the policies invariant to potential parameter error~\citep{sadeghi2016cad2rl, tobin2017domain,peng2018sim}. However, these policies are not \textit{adaptive} to unmodelled effects, i.e they take into account only aleoteric and not epistemic uncertainty. Also, such approaches are highly sensitive to hand-designed distributions used for randomizing simulation parameters and can be highly suboptimal on the real-systems parameters, for example, if a very large range of simulation parameters is used. Model-based approaches aim to use real data to improve the model of the system and then perform reinforcement learning or optimal control using the new model or ensemble of models~\citep{kurutach2018model, shyam2019model, ross2012agnostic}. Although learning accurate models is a promising avenue, we argue that learning a globally consistent model is an extremely hard problem and instead we should learn a policy that can rapidly adapt to experienced real-world dynamics. 

% Domain randomization (DR) aims to make policies learned in simulation invariant to potential parameter error by randomizing simulation parameters during training~\citep{sadeghi2016cad2rl, peng2018sim}. Such approaches are very sensitive to hand-designed distributions and can be suboptimal for modeling real variations, e.g. if a very wide range of simulation parameters is used or if the true parameters lie outside of the range. Model-based approaches use real data to improve the model of the system and then perform reinforcement learning or optimal control using it~\citep{kurutach2018model, shyam2019model, ross2012agnostic}. However, we argue that learning a globally consistent model is an difficult problem. Instead, we take the approach of learning a policy that can rapidly adapt to experienced real-world dynamics. 

% The use of entropy regularization has been explored in RL and Inverse RL for its better sample efficiency and exploration properties~\citep{ziebart2008maximum,fox2015taming,haarnoja2018soft,haarnoja2017reinforcement,schulman2017equivalence}. This framework allows incorporating prior knowledge into the problem and learning multi-modal policies that can generalize across different tasks. \citet{fox2015taming} analyze the theoretical properties of the update rule derived using mutual information minimization and show that this framework can overcome the over-estimation issue inherent in the vanilla Q-learning update. In the past,~\citet{todorov2009efficient} have shown that using KL-divergence can convert the optimal control problem into one that is linearly solvable. 

% Entropy regularization has been explored in RL and Inverse RL for its better sample efficiency and exploration properties~\citep{ziebart2008maximum,todorov2009efficient,fox2015taming,haarnoja2018soft,haarnoja2017reinforcement,schulman2017equivalence}. \citet{fox2015taming} analyze the theoretical properties of the update rule derived using mutual information minimization and show that this framework can overcome the over-estimation issue inherent in the vanilla Q-learning update. Infinite horizon MPC learns a terminal cost function to add global information to the finite horizon optimization.~\cite{rosolia2017learning} learn a control Lyapunov function and a safety set for the terminal state however they assume access to a controller that can deterministically drive any state to the goal.
%~\cite{tamar2017learning} learns a cost shaping to make a short horizon MPC mimic the actions produced by long horizon MPC offline. However, since their approach is to mimic a longer horizon MPC, the performance of the learner is fundamentally limited by that of the longer horizon MPC whereas learning an optimal value function as the terminal cost can potentially lead to close to optimal performance.

% Infinite horizon MPC aims to learn a terminal cost function that can add global information to the finite horizon optimization.~\cite{rosolia2017learning} learn a terminal cost as a control Lyapunov function and a safety set for the terminal state however they assume the presence of a controller that can deterministically drive any state to the goal.~\cite{tamar2017learning} learns a cost shaping to make a short horizon MPC mimic the actions produced by long horizon MPC offline. However, since their approach is to mimic a longer horizon MPC, the performance of the learner is fundamentally limited by the the performance of the longer horizon MPC. On the contrary, learning an optimal value function as the terminal cost can potentially lead to close to optimal performance. 



% Using local optimization is an effective way of improving an imperfect value function as noted in RL literature by~\cite{silver2016mastering,silver2017mastering,sun2018truncated,lowrey2018plan,anthony2017thinking}. However, these approaches assume that a perfect model of the system is available. In order to make the policy work on the real system, we argue that it is essential to learn a value function from real data and utilize local optimization to stabilize learning.
% Local optimization is an effective way of improving an imperfect value function as noted by~\cite{silver2016mastering,silver2017mastering,sun2018truncated,lowrey2018plan,anthony2017thinking}. However, these approaches assume that a perfect model of the system is available, which is not the case when dealing with robotic systems. Hence, we argue that it is essential to learn a value function from real data and utilize local optimization to stabilize learning.

